DiscoveryBench: Towards Data-Driven Discovery with Large Language Models

Can the rapid advances in code generation, function calling, and data analysis using large language models (LLMs) help automate the search and verification of hypotheses purely from a set of provided datasets? To evaluate this question, we present DiscoveryBench, the first comprehensive benchmark that formalizes the multi-step process of data-driven discovery. The benchmark is designed to systematically assess current model capabilities in discovery tasks and provide a useful resource for improving them. Our benchmark contains 264 tasks collected across 6 diverse domains, such as sociology and engineering, by manually deriving discovery workflows from published papers to approximate the real-world challenges faced by researchers, where each task is defined by a dataset, its metadata, and a discovery goal in natural language. We additionally provide 903 synthetic tasks to conduct controlled evaluations across task complexity. Furthermore, our structured formalism of data-driven discovery enables a facet-based evaluation that provides useful insights into different failure modes. We evaluate several popular LLM-based reasoning frameworks using both open and closed LLMs as baselines on DiscoveryBench and find that even the best system scores only 25%. Our benchmark, thus, illustrates the challenges in autonomous data-driven discovery and serves as a valuable resource for the community to make progress.

==> sections/4_discovery_agents.tex <==
\section{Experiments}
\label{sec:discovery_agents}
We benchmark state-of-the-art LLM-based few-shot reasoning methods as discovery agents with two closed models, GPT-4o and GPT-4-0125-preview (GPT-4p), and one open, Llama-3-70B, model powering the reasoning methods. A discovery agent takes the task description, paths to the task dataset(s) $D$, metadata about the datasets (description, column descriptions), and the goal, $G$, to produce a natural language (NL) hypothesis specified by context, variables, and relationship. 

% \textbf{Output format:} an NL hypothesis + (optional) used workflow in NL

% \begin{itemize}[left=2pt, itemsep=0.1pt]
\begin{ite}
    \item \textbf{CodeGen} generates the entire code at one go to solve the task, where we provide a demonstration of a solution code in the context. After code execution and based on the result, it generates the NL hypothesis and summarizes the workflow.
    \item \textbf{ReAct} \cite{yao2023react} solves the task by generating thought and subsequent codes in a multi-turn fashion.
    % code-generation and ability to solve the task. For each turn, the agent generates a "think" statement followed by a Python code. Upon executing code, the system performs a think $\rightarrow$ code generation loop till it thinks it has solved the task. Otherwise, we cut off after a fixed step limit.
    \item \textbf{Reflexion} \cite{Shinn2023ReflexionLA} is an extension of CodeGen agent, where at the end of one trial, we provide the oracle HMS score as an evaluation signal, and it generates a reflection to improve (when $\mathrm{HMS} < 1$) in the next trial till it solves the task, or maximum trials (3) are reached.
    % We extend the Base agent with reflection capability. After one (only) step of code execution and final hypothesis generation, we allow the agent to reflect if the answer is not correct (oracle reward). Then, we restart the agent to solve the task again, but along with the input, the additional reflection is provided to the agent.
    \item \textbf{DataVoyager} is a multi-component data-driven discovery agent, introduced in \cite{majumder2024data}. It has four components, planner, code generator, data analysis, and critic, that orchestrate the discovery process.
    % \item \textbf{ReAct + Reflexion:} Now we replace the Base agent with the ReAct agent in the previously discussed Reflexion agent---this now has the ability to think while solving the task and reflect at the end of the task.
\end{ite}
% \end{itemize}

% \textbf{Experiments}
% Results from the running discovery agents on DiscoveryBench.

% \textbf{API-based:} GPT-4o, GPT4-0125-preview, \textbf{Open} Llama-3


% \textbf{Zero-shot vs. Few-shot:}

% \subsection{Single-agent Frameworks}
% Supported models: Claude, Llama, Gemma, OLMo, Gemini (with diff features like code-llama); Supp. prompts: ReAct, Plan-and-Execute, Retry


% \subsection{Multi-agent Frameworks}
% Supported models: GPT-4, 3.5, turbo; Supp. prompts: ReAct, Plan-and-Execute, Retry

==> sections/6_related_work_v1_old.tex <==
\section{Related Work \pete{WIP}}
\label{sec:related_work}

\cite{majumder2024data}
TBA.

\newpara{End-to-end Data-driven Discovery.} 
Most previous autonomous data-driven discovery systems, such as Bacon \citep{Langley1981DataDrivenDO, Langley1984TheSF, Langley1983RediscoveringCW} severely lacked the requisite computational power, restricting their scope with limited discovery of data-driven knowledge. A recent system, CoScientist \citet{Boiko2023AutonomousCR}, uses LGMs to automate some parts of the workflow; however, it still requires substantial human intervention (e.g., wet lab experiments) for hypothesis verification, thus not qualifying as a fully autonomous discovery system. DataLume \cite{Gu2023HowDD} fully automates the code generation for data transformation and hypothesis verification; however, do not support hypothesis search for complex science workflows. \citet{Gil2022TowardsCS, Gil2017TowardsCS, Gil2013UsingSW} as well as Automatic Analysis in WolframAlpha\footnote{\url{https://www.wolframalpha.com/examples/pro-features/data-input}} prototyped various workflows for conducting science in data-driven ways, however, such prototypes never explored the power of LGMs and are only exhibit limited generalizability to datasets and scientific methods. 

% CoScientist, Bacon, DataLume, Mathematica \harshit{Structure: Can be covered in this flow: [Bacon as the foundational system. Attempts by Mathematica. Then domain-specific attempts by Coscientist and DataLume.][Q: shall we also cover other attempts for doing science by DeepMind and MSFT at the start? I don't think any of them are end-to-end though. Or their coverage in the intro suffice? ]}

\newpara{AutoML.}
AutoML is a workflow of automatically building optimal machine learning and predictive models. AutoML tools exist in scientific packages like Scikit \cite{feurer2015efficient} and also in cloud platforms such as Google Cloud Platform\footnote{\url{cloud.google.com/automl}}, Microsoft Azure\footnote{\url{azure.microsoft.com/en-us/products/machine-learning/automatedml/}}, and Amazon Web Services\footnote{\url{aws.amazon.com/machine-learning/automl/}}. Existing AutoML Cloud platform systems primarily
% mainly focus on black box models, ensuring the models can be served at scale. Despite 
perform search over hyperparameters for optimal model development, but they cannot comprehend the semantics of the data and hence cannot help with data-driven hypothesis generation, orchestrating research pathways, and knowledge integration. MLAgentBench \cite{Huang2023BenchmarkingLL}, an evolution of AutoML, performs end-to-end machine learning to benchmark AI research agents. MLAgentBench can plan, evaluate hypotheses, and measure progress, but with a focus on optimizing machine learning models, not on discovering new and novel scientific knowledge.


% Google AutoML, MLAgentBench, AutoGluon/AWS Sagemaker, AutoML from other groups \harshit{Structure: AutoML tools exist in scientific packages like Scikit (link) and also in cloud platforms on Google Cloud Platform, Microsoft Azure and Amazon Web Services. Cloud platform systems like Google AutoML focus on black box models while ensuring the models can served at scale. MLAgentBench can be considered as an evolution of AutoML that does end-to-end ML to benchmark AI research agents. General AutoML tools can only help partially with hypothesis evaluation and measurement of progress. The cloud platforms tools can work on large datascale. But outside of this they do not help with hypothesis generation, planning and orchestrating research pathways and knowledge integration - something the ideal DDD system can do. MLAgentBench can plan, evaluate hypothesis and measure progress, but with a focus on optimal models, not for discovering new and novel science.}

\newpara{Automated Data Analysis.}
Automated Data Analysis tools are primarily focused on exploring data under a user-provided query (e.g., ``plot sales trends for last 12 months'', etc.) and often do not have the capability of searching through the hypotheses space as defined by the data.
% Tools such as PowerBI\footnote{\url{https://www.microsoft.com/en-us/power-platform/products/power-bi}}, Tableau\footnote{\url{https://www.tableau.com/}}, and Thoughtspot\footnote{\url{https://www.thoughtspot.com/}} can, however, perform multi-step hypothesis verification using inbuilt data transformation and statistical tools, though the interpretation and consumption of such analysis are left to the user.
Spreadsheet tools such as Microsoft Excel and Google Sheets are often part of the scientific workflow as the data analysis tool but show limited automation ability even after coding (Python) support \cite{PYExcel, duetai}. Focus on integrating LGMs into data analysis with known workflows \cite{Perlitz2022nBIIGAN, Chakraborty2024NavigatorAG}  and code-first data analysis \cite{ydata} increased recently---however, these are limited to small-scale tables and lack abilities such as orchestrating research plans, interpreting results, and knowledge integration. 
